Cloud Watching: Understanding Attacks Against Cloud-Hosted Services

Cloud computing has dramatically changed service deployment patterns. In this work, we analyze how attackers identify and target cloud services in contrast to traditional enterprise networks and network telescopes. Using a diverse set of cloud honeypots in 5~providers and 23~countries as well as 2~educational networks and 1~network telescope, we analyze how IP address assignment, geography, network, and service-port selection, influence what services are targeted in the cloud. We find that scanners that target cloud compute are selective: they avoid scanning networks without legitimate services and they discriminate between geographic regions. Further, attackers mine Internet-service search engines to find exploitable services and, in some cases, they avoid targeting IANA-assigned protocols, causing researchers to misclassify at least 15\% of traffic on select ports. Based on our results, we derive recommendations for researchers and operators.

==> scraps/conclusion.tex <==
\section{Conclusion}
\label{sec:rec_conclusion}


\todo{add conclusion}
Attacker behavior today is more selective and sophisticated than what the majority of prior work has assumed. 

Preparing for next gen of security papers.






==> scraps/intro_scraps.tex <==

%Network intrusion attacks have become constant and ubiquitous.\todo{I think you could add a few citations here. It's 100\% true but there are easy cites to back you up.}
%from nation-state actors to amateurs targeting governments~\cite{costa_ransom}, companies~\cite{business_ransom}, hospitals~\cite{hospital_ransom}, and individuals~\cite{mirai}.
%By exploiting vulnerabilities found through Internet scanning, attackers have successfully extorted 20~billion dollars~\cite{ransomBillions}, shut down a major gas pipeline~\cite{colonialPipeline}, cut off a country's electric grid~\cite{ukrainePowerGrid}, and increased hospital mortality rates~\cite{mortality}. 
%As a result, the security research community has prioritized
%To help save lives, infrastructure, and money, the security community has relied on 
%accurately detecting and understanding malicious Internet scanning.\todo{feels weird to end here without any citations or supporting evidence. It's in the next paragraph, but it's awkward to paragraph break here. Part of me wonders if this sentence is better suited for the next paragraph.}




%\todo{cite UK securing services?}
%\todo{It's a strange transition to go from ``recently'' to ``last 20 years''. What's the bridge?}
%Over the past two decades, researchers have used network telescopes (i.e., darknets)---large swaths of unused IP address space~\cite{2004-moore-t20}---to understand malicious behavior including botnet infiltration~\cite{mirai,malecot2013carna}, worm propagation~\cite{singh2004automated,irwin2013source}, and DDoS attacks~\cite{nawrocki2021far,kramer2015amppot}.
%In the last year alone, researchers have used network telescopes in over a dozen of papers \todo{Split the papers to organize them by topic, i.e., used telescopes to do what? +1 -ZD I would merge this was the sentence prior and say that in the last year alone people have used them to X, Y, Z. You don't need to have both.}~\cite{griffioen2021scan, spoki,nawrocki2021far,han2022dark,nader2022attentive,demertzis2021darknet,houmz2021detecting,sarwar2021darkdetect,pourhoneycomb,nishijima2021verification,liu2021ipv6,kallitsis2021zooming,cabana2021threat,rawat2021analysis,2021-mayerhofer-pmt1,2021-goldschmidt-igv82,2021-saha-ssl1,2021-pour-pmi0,2021-panigrahi-prm9,prajapati2021shedding}. 
%In the last year alone, researchers have used network telescopes in more than 20 papers. These papers continue to study DDoS attacks~\cite{2021-goldschmidt-igv82,griffioen2021scan,nawrocki2021far,2021-saha-ssl1} IoT bots~\cite{nader2022attentive,2021-pour-pmi0,pourhoneycomb} and the general darknet ecosystem and state of the internet~\cite{spoki,liu2021ipv6,2021-mayerhofer-pmt1,nishijima2021verification,prajapati2021shedding} although a common trend among these papers is to develop and employ more sophisticated methods like applied machine learning to detect malicious activity in darknets~\cite{demertzis2021darknet,2021-goldschmidt-igv82,han2022dark,houmz2021detecting,kallitsis2021zooming,2021-panigrahi-prm9,2021-pour-pmi0,rawat2021analysis,2021-saha-ssl1}.
%However, over the years the majority of services have migrated away from the networks that house telescopes and to the public clouds~\cite{censys_hosts}.\todo{Not really sure how you got this from the cite. I also don't think it's true. Nothing was ever on these networks, especially when they're an unpopulated /8. I get what you're saying, there's a migration from on-prem to and a higher density of services in cloud, but you need to be more specific here.}
%Cloud computing has provided increased service deployment options---customers can choose from a myriad of networks and geo-locations---at the expense of heavily recycling IP address space---services are often assigned a random IP address previously used by a different service. 
%Today, the attack surface of Internet services is distributed across a myriad of network operators, geo-locations, and a heavily recycled IP address space. 



\todo{Missing 1 sentence for motivation/scope}
\todo{I think that this is an over claim. It comes across as how attacks choose any services to attack, you're looking at something more specific}
In this work, we empirically investigate how, within today's heavily distributed and recycled Internet service ecosystem, scanners choose and attack services.
\todo{Missing 1 sentence about why is this important / why should folks care, this could actually be the last sentence of the intro going here}
We use a diverse set of perspectives representative of the modern Internet, 8 networks (5~cloud, 2~educational, 1~telescope) across 23~countries.\todo{is it really representative when you are missing the majority cases like ISPs and Businesses?} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%
Network intrusion attacks are widespread and the new normal, contributing towards distributed denial of service attacks, ransomware attacks, etc. \todo{cite logjam}
To prevent service exploitation, operators often focus on securely configuring the transport layer (e.g., tls), application layer (e.g., key authentication), and, more recently, hardware (e.g., sgx).
With the rise of cloud computing's popularity, operators now also have the ability to decide where should the location (i.e., IP address, geographic region, network) of a service be hosted. 
However, the location of a service is rarely factored in as a means to  more securely configure a service, and is rather more commonly chosen  based on expected network performance (e.g., selecting a close geographic region to the clients), cost (e.g., selecting the cheapest cloud computing network), or random choice (selecting a random IP address within a network to host the service).
For example, is a service located in an educational network more or less likely to be the target of a network scan compared to the same service being hosted by Google in the same geographic region?


%While, anecdotal evidence has shown that scanners and attackers discriminate amongst entire network and geographies (e.g., UK's National Cyber Security Center conducting scans of UK services~\cite{uk_scanning}, Russian malware avoiding Russian services~\cite{russian_keyboard}), it is not clear 

==> scraps/protection.tex <==
\section{Evaluating Blocklist Efficacy Against Network Scanning}
\label{sub:sec:blocklists}
To protect networks from malicious network scanners, companies and network operators often compile and share seemingly malicious IP addresses and payloads, often through the form of blocklists and firewall filters. 
Relying on blocklists and filters assumes that (1) Attackers are indiscriminately attacking networks (i.e., malicious traffic and traffic origins seen by one network will likely be seen by another) (2) The same attackers /attacks return (i.e., blocklists and filters are effective at pro-actively filtering traffic). 

Rely on outside sources that curate lists with unknown methodologies and secret network of sensors. 




\subsection{Location of Sensors}

Darknet vs not. 

\subsection{Impact of Protocol}

Protocol affects the likelihood of sensors seeing similar traffic: sensors are 2x as likely to see the same sourceIP if it is scanning for the SSH protocol, as opposed to Telnet. We discuss the cause of this phenomemon in detail Section~\ref{sub:sub:ssh_v_telnet}, where we show that this is due to SSH scanning actors are more likely to scan more unique IP addresses. 
Telnet username and passwords are more likely to be repeated sin

ce Telnet scanning actors are 3x more likely to attempt multiple login credentials compared to scanners attacking the SSH protocol. 


\textbf{Temporal Efficacy}
Impact of port, protocol, location, and temporal nature of scanning IPs. 

%Due to a protocol's often unique attackers and therefore different attacker behavior, the protocol being scanned for directly affects the probability that the same source IP address will re-appear to launch an attack and thus the efficacy of blocklisting IP addresses.
Blocklisting IP addresses is one of the most common ways network operators filter malicious traffic \todo{cite}. While previous work has demonstrated the harm in blocklisting IP addresses--- as it can likely block benign users who are NATed behind the same address~\cite{ramanathan2020quantifying}---and prior work has worked to find better ways to identify attackers \todo{cite}---blocking individual IP addresses is still one of the most widely-adopted method to identify and block scanning traffic \todo{cite}.
\label{sub:sub:ssh_v_telnet}

The SSH and Telnet protocols are targeted by scanning actors with fundamentally different scanning patterns and behaviors, which complicates the efficacy of blocklists. 


Scanners attacking Telnet are over 3x more likely to attempt multiple login credentials compared to scanners attacking the SSH protocol (Figure~\ref{fig:sshTel_login}) across all cloud provider sensors (Table~\ref{table:data_breakdown}). While 78\% of unique SSH attacking source IPs only attempt one login per sensor across the entire week, 60\% of unique Telnet attacking source IPs attempt at least ten logins per sensors.  
While SSH attackers are less likely to attempt multiple login credentials per one sensor, they are more likely to target more sensors Internet-wide. On average, an SSH attacker targets 3~times the amount of unique regions within a cloud provider, and 3~times the amount of unique (Figure~\ref{fig:ssh_target} and Figure~\ref{fig:telnet_target}). 

%In reality, these are small sub-sampled scan.  Telnet: 98\% and 90\%  of all source IPs only scan 1/4 sensors within a region for Telnet and SSH, respectively. 


  
 
\begin{figure}[h]
  \includegraphics[width=\linewidth]{fig/sshTel_logins_cdf.pdf}
  \caption{\textbf{Login Attempt}---% The number of
  Scanners attacking Telnet are over 3x more likely to attempt multiple login credentials compared to scanners attacking the SSH protocol. 
	} \label{fig:sshTel_login}
\end{figure}

\todo{grab key data from figs, get rid of source IP figs. }
Within 1 week, a sensor never sees traffic coming from 77\% of all source IPs that send malicious traffic to the service on day~1 (Figure~\ref{fig:sourceIP_where}). Furthermore, 92\% of all source IPs do not scan the same sensor for more than 1~day. 
However, source IPs are much more likely to re-appear scanning other sensors. Only 6\% of source IPs send traffic only once, and 35\% of source IPs scan other sensors across the week. 
This is likely due to teh byproduct of scanners visiting a random sub-set of the IP address space as opposed to target region/cloud-wide scans. 


\begin{figure}[h]
  \includegraphics[width=\linewidth]{fig/ssh_TargetAppearance_cdf.pdf}
  \caption{\textbf{Source IP Appearance}---% The number of
  \todo{todo}
	Source IPs are unlikely to target the same sensor within 1 week and are rather more likely to target a sensor in a completely different cloud provider.  
	} \label{fig:sourceIP_where}
\end{figure}

\begin{figure}[h]
  \includegraphics[width=\linewidth]{fig/telnet_TargetAppearance_cdf.pdf}
  \caption{\textbf{Source IP Appearance}---% The number of
  \todo{todo}
	Source IPs are unlikely to target the same sensor within 1 week and are rather more likely to target a sensor in a completely different cloud provider.  
	} \label{fig:sourceIP_where}
\end{figure}

% sql: max time - min time 
\begin{comment}
% # filt for day 1only mal (ssh/telnet) max time - min time : by metatype (isp, hosting) target_ip
% with label as (
% SELECT distinct metadata.org org, metadata.type t
% FROM `orion-20191028.greynoise.gn_rorschach_view` 
% ),
% alldata as (
%   SELECT t1.*, t FROM
%   (SELECT provider, region, source_ip, target_ip, timestamp, org
%   FROM `orion-20191028.greynoise.gn_ssh_view` 
%   where meta_type = "cowrie.login.failed" )t1
%   INNER JOIN
%   (SELECT org, t FROM label)t2
%   ON t1.org = t2.org
%   UNION ALL
  
%   SELECT t1.*, t FROM
%   (SELECT provider, region, source_ip, target_ip,  TIMESTAMP_SECONDS(timestamp), org
%   FROM `orion-20191028.greynoise.gn_telnet_view` 
%   where meta_type = "cowrie.login.failed" )t1
%   INNER JOIN
%   (SELECT org, t FROM label)t2
%   ON t1.org = t2.org
% ),
% filtdata as (
% SELECT t1.* FROM
% (SELECT * FROM alldata)t1
% INNER JOIN
% (SELECT distinct source_ip FROM 
% `orion-20191028.greynoise.gn_telnet_view` 
%   where meta_type = "cowrie.login.failed"  and EXTRACT(DAY from TIMESTAMP_SECONDS(timestamp)) = 1
%   UNION ALL 
% SELECT distinct source_ip FROM 
% `orion-20191028.greynoise.gn_ssh_view` 
%   where meta_type = "cowrie.login.failed"  and EXTRACT(DAY from (timestamp)) = 1 )t2
%   ON t1.source_ip = t2.source_ip
  
%   )
% SELECT q FROM (
% SELECT APPROX_QUANTILES(c,100) qs FROM ( 
% SELECT source_ip, t, target_ip, TIMESTAMP_DIFF(MAX(timestamp), MIN(timestamp), SECOND)/60/60  c
% FROM filtdata
% GROUP BY source_ip,t ,target_ip
% )),UNNEST(qs) as q
\end{comment}






==> scraps/related.tex <==
\vspace{3pt}
\todo{OLD SECTIONS}


\vspace{3pt}
\noindent
\textbf{Honeypots in the Cloud.}
We present, to the best of our knowledge, the most geographically diverse, network diverse, and statistically rigorous empirical investigation of attacker traffic across cloud vantage points. 
%Nevertheless, there has been little statistical-rigor and investigation into the broader patterns of what IP addresses, network types---beyond telescopes---and geographic regions attackers target. 
Recent work~\cite{kelly2021comparative,brown2012HoneypotsIT,bove2019} directly compares scanning traffic across cloud providers, but, as we show in this work, use an inaccurate methodology (e.g., use only one honeypot per region, no statistical validation) that is likely only measuring noise.
\todo{maybe resurrect the sentence we used to have about what one of those works found/did}
\todo{add more related work in this paragraph? other cloud papers?}
The simplicity of renting virtual machines in different geographic locations has also been utilized when studying automated bots~\cite{griffioen2021scan} and DDoS attacks~\cite{li2021good}.  
\gn (anonymized for submission), a company whose mission is to collect and label all security-critical Internet traffic, also deploys honeypots across many cloud providers and geographic locations. %~\cite{greynoise_company}

\vspace{3pt}
\noindent
\textbf{Telescopes.}
Hundreds of research papers have used network telescopes and darknets~\cite{caida_catalog} to understand Internet background radiation~\cite{wustrow2010internet,pang2004characteristics}, malicious scanning patterns~\cite{irwin2013baseline,irwin2013source,chatziadam2014network,pang2017malicious}, DDoS attacks~\cite{nawrocki2021far,kramer2015amppot}, worms~\cite{singh2004automated}, and botnets~\cite{mirai,torabi2020inferring}.
We are the first work, to the best of our knowledge, to compare cloud- and telescope-targeted scanning attacks. \todo{manda: is that true? }


To ensure scientific validity, researchers have extensively studied the caveats of telescope deployment: understanding how the size~\cite{moore2002network}, network~\cite{soro2019darknets}, and geographic location~\cite{irwin2013baseline,spoki,pham2011honeypot,pouget2005advantages,soro2019darknets} of darknets change research results. 
% The expansive address space that network telescopes provide has been crucial to studying temporal and spatial scanning behavior~\cite{durumeric2014internet}.
In 2019, Richter et~al.\ showed that there are significant differences between the scans that target darknets and a content delivery network~\cite{richter2019scanning}, and Huston highlighted that network telescope traffic has dramatically shifted away from targeted malware scanning~\cite{dark_traffic}.
\todo{(is this true manda??)}
Further, we show that all popular telescopes, except for Spoki~\cite{spoki}, which do not collect payloads, mistakenly assume that scans primarily target IANA-assigned protocols.  



==> scraps/scraps.tex <==


%Variation in attacker behavior impacts the ability of network intrusion systems to uniformly protect neighboring services across different threats. 
%On average, Suricata identifies the maliciousness of an HTTP/80 payload with 91\% accuracy, relative to our ground truth (Section~\ref{sub:sec:suricata}).
%Suricata accuracy varies significantly amongst neighboring honeypots (small $\phi$=0.15).
% with a 6\% variance in accuracy and,
%In the worst case, Suricata is 15\% less accurate across honeypots within the Azure South-East Asia region, failing to identify the maliciousness of payloads attempting to spawn a shell. 

\subsection{What fraction traffic is not scanning for the assigned protocol?}

Filter for traffic that sends data.


Recent work showed that the majority of services live on unassigned ports and that, as ports become less popular, the fraction of unassigned services dramatically increases~\cite{lzr}. 

23/SSH:0.0001\%
23/HTTP: 0.08\%
23/FTP: 0.09\%
2323/SSH:0.008\%
2323/FTP:0.4\%
2323/HTTP: 6.8\%

TLS events discarded...


\todo{finish analysis/figure with remaining data}
\todo{are tls events more likely to have malicious data}


Alternative ports are more likely to be scanned the unassigned protocol.


2323/benign/unexpected 42\% 
23/benign/unexpected 39\%

23/benign/sending data = 0.0005\% 
2323/benign/sending data = 3\% of all traffic. 

Unexpected protocol ~5 orders of magnitude more likely to be scanned by a classified benign actor than the expected protocol.


Port 22 and 2222 are excluded in the analysis due to Greynoise's collection method. Their collection method assumes that the protocol being scanned is assigned, and therefore does not accomodate this analysis. 







\section{Attacker Rationality}

In this section we explore which attackers  maximize expected probability of compromise?

Are attackers more or less incentivized to "attack" clouds? Does it make more or less sense to "attack" the clouds? 

Key auth vs brute force. certain clouds are more likely to be using one over the other. Are attackers aware of this

Random password per host vs static password. What’s more common—statistically speaking, should use the same popular passwords (birthday paradox) but zakir claims there is some logic behind why botnets will rotate passwords

Should attackers actually try different language passwords? (Is foreign content more likely to be served in certain regions..can use as a proxy) (Chinese passwords paper, shows they are different)


Do attackers use censys to attack? VMs with open services vs not. 


%%%%%%%%
Sensors set-up primarily comes in two configurations: honeypots \todo{cite} and darknets \todo{cite}.
While darknets often span large swaths of IPv4 address space (e.g., the CAIDA darknet uses a globally routed /8 network~\cite{caidaTel}), honeypots are assigned to fewer IP addresses, due to the server resources needed to upkeep server interaction~\todo{cite}. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Characterizing Scanning Traffic}
\label{sub:sec:characterizing_traffic}

We identify the primary attributes of scanning traffic that we use to comprehensively understand and compare targeted network scanning. 

\textbf{Who.} 
%The IP address is the most common---and most simple to obtain---identifier of a network scanner  \todo{cite prior work which uses ip addresses to figure out who is scanning...literally like all prior work}. The IP address scanning identifier is also the most commonly used attribute to block likely-malicious traffic, through the use of blocklists. 
We use the IP address to identify scanning actors, as well as the autonomous system of the scanning actors in order to accommodate identifying scanning organizations that often rely on multiple IP addresses to conduct scanning campaigns (e.g., Censys~\todo{cite}) and the prevalence of sub-sampled scanning~\cite{durumeric2014internet},
%\todo{Mention prior work fingerprinting who but how our datasources do not offer such capabilities.}

\textbf{What.}  We focus our results on three popular protocols: the most popular protocol used by botnets~\cite{mirai}, Telnet, and the two protocols responsible for over 90\% of ASCII payloads sent by network scanners~\cite{spoki}: HTTP and SSH.
%ASCII payloads comprise the majority of payloads, according to spoki

\textbf{Where.} 
Prior work \todo{cite akamai paper, leurre} has shown that ``sensors'' within different networks and/or geographic locations experience different incoming scanning traffic. 
 
We cosndifferent facets of a service's location: IP address, port, geographic location, network. Furthermore, we also consider 


\textbf{When.} (Time Zone?) Time of compromise. 



\textbf{Why.}
Multiple motivations exist behind un-solicited network scans; for example, individuals or organizations conducting benign research, malicious actors actively exploiting a service, malicious actors performing reconnaisance with the intent of later exploitation, etc. 
Understanding the true intent behind a network scan is often challenging: Greynoise is a company dedicated to understanding the intent behind network scans and \TK \% of the IPs Greynoise labels are classified as ``unknown.'' 
Thus, prior work that studies network scanning often assumes that the majority of inbound scanning traffic is security-critical \todo{Manda, can you find like 5 example papers here and cite them? any paper that uses a darknet (e.g., CAIDA, or Orion Network Telescope) will likely assume this (b/c darknets dont collect payloads..)}
In this work, we account for the fact that not all network scans may be security-critical, by using the payload(s) of arriving scanning traffic to classify the maliciousness of the scan. 
Concretely, we define a malicious payload to be one that either (1) attempts a login (2) attempts to alter the state of the service (e.g., running a shell command). 
We detail our exact methodology for identifying malicious payloads in Section~\ref{sub:sec:intrusion_detection}. 

\textbf{How.} (Top Payloads) - usernames/passwords. HTTP payloads
The most common payloads received (after removing the Host, Content-Length, and Date header fields, when applicable)



\textbf{Volume.} Risk of being targeted. Time To Compromise ?

%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsubsection{Categories of malicious IPs}


\todo{mention botnets (characteristics of source IPs) vs not}
The organizations that house SSH scanning IPs are Top 10 source IP organizations make up 15\% of SSH source IP versus 43\% for Telnet. 
Nonetheless, there 2~times the unique number of organizations scanning Telnet compared to SSH. 
Hosting providers dominate the most popular SSH scanning organizations (Shenzhen Tencent, Digital Ocean and Alibaba and Amazon being in the top 10 organizations), whereas all top 10~telnet organizations are Telecoms or ISPs. This is unsuprising, as botnets, which often use the Telnet protocol (e.g., Mirai~\cite{mirai}),  often rely on IoT devices which are more likely to be found in non-hosting provider networks. 




Attackers can easily change IPs, which further complicates the efficacy of blocking IP addresses. 

81\% of source IPs used belong to an ISP network, 14\% belong to a hosting provider 4.4\% to a business provider and, interestingly, 0.1\% to an education network (predominantly located in \TK). We further identify 0.05\% of all source IPs are mapped to known Tor exit nodes. 
Source IPs belonging to a hosting provider are actually 2x more likely to exploit another sensor after the majority of the week has elapsed, compared to a source IP belonging to an ISP. 
In our dataset, 48\% of source IPs that reappear after over half the week has elapsed belong to a cloud owned by Shenzhen Tencent Computer Systems, and 18\% belong to Digital Ocean, both of which predominantly host legitimate clients (i.e., are not bullet proof hosters). Due to the ease at which an attacker can request a new IP address and a benign user could unbenowingly obtain the previously-owned attacker IP address, blocklisting is more likely to unintentionally block legitamite traffic.
\todo{cite some proof of churn}

Shenzhen Tencent (20.7\%) , China Unicom (7\%) , and Chinanet Backbone (3\%) make up 35\% of source IPs mapped to ISP that are most likely to return within the week. \todo{are they known for NATing their IPs?}


\textbf{Look into education network scanning events as a fun case study}
\todo{evaluate greynoise blocklist?}



%%%%%%%%%%%%%%%%%%
\subsection{HTTP Classification Methodology}
\subsubsection{Re2Pcap}
Re2Pcap is a tool developed by Cisco to convert raw HTTP Requests to Pcap Files.

% Links: 
% https://github.com/Cisco-Talos/Re2Pcap, https://talosintelligence.com/re2pcap, 
% https://doc.emergingthreats.net/bin/view/Main/AllRulesets

\subsubsection{Suricata}
"Suricata is a high performance Network IDS, IPS and Network Security Monitoring engine. It is open source and owned by a community-run non-profit foundation, the Open Information Security Foundation (OISF). Suricata is developed by the OISF."

In order to minimize the total number of HTTP payloads processed without losing important information we removed the Host headers when determining the distinct payloads. To identify malicious traffic over HTTP we converted the distinct HTTP payloads into pcap files using Re2Pcap, a tool developed by Cisco. We tested the generated pcap files against the Suricata base ruleset. By parsing the Suricata logs by timestamp we matched the timestamp of the Suricata alert with the timestamp of the pcap using tcpdump. 

The Suricata base ruleset was altered to allow alerts from all ip addresses and all ports by modifying all rules to allow `any` source and destination ip addresses and ports. We disregarded source and destination IPs from the ruleset because the pcap files generated from Re2Pcap have default source and destination ip addresses 10.10.10.1 and 172.17.0.2 respectively. Additionally we wanted to minimize false negatives by removing blacklisted ip-based rules. We ran Suricata using both the base ruleset with ports and without ports. We found that only 12 alerts out of 319 alerts differ in the number of unique payloads that triggered the alert. Each of the 12 alerts reported a greater number of unique payloads when the rules excluded ports than when the rules included. We manually identified that only three out of the 12 alerts could be attributed to malicious activity (i.e. remote code execution or attacks). After manually checking the difference between the payloads caught by the ruleset without ports, but missed by the ruleset with ports, we were still able to manually classify the payloads as malicious. Thus we decided to use the dataset generated by the ruleset without ports and without ip addresses in order to gain more coverage.

168577 pcap files (of distinct payloads without Host header) were generated using Re2Pcap. We will refer to the number of generated pcap files as the number of distinct payloads.

The count HTTP payloads in the GreyNoise dataset was: 10,516,191 (verify that this number makes sense with the ssh/telnet numbers, there should be a total count of 67,999,984 over both weeks).

The base ruleset in Suricata contains 24,216 rules. (There are 31,590 in the suricata\_rules\_all dataset but some of the alerts were commented out)

319 rules from the base ruleset were triggered when running Suricata on our GreyNoise pcaps.

Out of the 319 rules, 134 rules were classified as semi-malicious or malicious. Here we define semi-malicious as any access or attempted access to private data, unencrypted passwords, etc and we define malicious as attempted or successful remote code execution or injections and upgraded/bypassed authority. 90 rules were identified as malicious and 44 semi-malicious.

Using the manually identified semi-malicious and malicious alerts as the criteria for malicious HTTP activity, we find that 10,244 (6.0767\%) of the distinct payloads are malicious and 150,996 (1.4358\%) out of the total number were malicious.

After analyzing the >85\% of distinct payloads that did not trigger a malicious alert, we found 54 distinct payloads out of the 229 payloads that were manually checked could be attributed to malicious HTTP requests. Out of the total number of non-maliciously alerted payloads, 2,657,793/6,791,659 (39.1332\%) were false negatives. 


Also came to the conclusion that filtering by classtypes is not a good idea. Too many false positives and false negatives.

Suricata Conclusion: It is useful if you carefully pick and choose the rules you want to include, and if you write rules that are specific to your system.

%give number before looking at content (using classtypes in suricata)
When filtering by classtypes in Suricata:\\
If you include the following classytpes: 
\begin{verbatim}
['suspicious-login','rpc-portmap-decode','denial-of-service','successful-admin',
 'external-ip-check','suspicious-filename-detect','attempted-dos','successful-dos',
 'attempted-recon','attempted-user','misc-attack','credential-theft',
 'command-and-control','coin-mining','successful-recon-limited','exploit-kit',
 'pup-activity','domain-c2','web-application-attack','shellcode-detect',
 'default-login-attempt','successful-recon-largescale','attempted-admin',
 'protocol-command-decode','trojan-activity','successful-user',
 'unsuccessful-user','bad-unknown','web-application-activity',
 'targeted-activity','system-call-detect']
 \end{verbatim}
 
 We found that 16,913 (0.100328) unique payloads were classified as malicious and 239,217 (0.022747) in total were classified as malicious.

% give classtype and give dumb example of what it's matching on
Examples of rules that were classified as "non-malicious" - too vague
\begin{enumerate}
    \item 
        \begin{verbatim}
            alert http $HOME_NET any -> $EXTERNAL_NET 443 
            (msg:"ET POLICY HTTP traffic on port 443 (POST)";
            flow:to_server,established; 
            http.method; 
            content:"POST"; 
            http.header; 
            content:!".etrade.com|3a|443|0d 0a|"; 
            classtype:bad-unknown; 
            sid:2013926; 
            rev:9; 
            metadata:created_at 2011_11_18, updated_at 2020_05_12;)
        \end{verbatim}
    \item
        \begin{verbatim}
            alert http $EXTERNAL_NET any -> $HTTP_SERVERS any 
            (msg:"ET INFO User-Agent (python-requests) Inbound to Webserver"; 
            flow:established,to_server; 
            http.user_agent; 
            content:"python-requests/"; 
            classtype:attempted-recon; 
            sid:2017515; 
            rev:6; 
            metadata:created_at 2013_09_25, updated_at 2020_09_13;)
        \end{verbatim}
\end{enumerate}



% do we expect regional differences in these numbers?
%   intuitively, not super interesting
%   do diff regions get statistically significant different payloads

% TODO: upload cleaned, manually labeled rules
%       cleaned regional dataset to query: `darknet-collab.greynoise.suricata_by_region_manual_class`
%       darknet dataset (raw pcaps) assumption that scanning is uniform random. given darknet and ip addresses 

% fraction of malicious, benign, and semi-malicious: split out fractions
% TODO: split out by week, 
%   was HE across both weeks?

% put suricata stuff on pause

% hurricane electric are they rolling across days or spikes?
% when comparing regions, do regions/ip's do we include random spikes

% calculate false positive do calculations per region and per provider 6.2. Intrusion Detection
% https://romisatriawahono.net/wp-content/uploads/2013/01/Liao-Intrusion-detection-system-A-comprehensive-review-2013-.pdf
% https://www.spiedigitallibrary.org/conference-proceedings-of-spie/8757/875704/Quantitative-analysis-of-intrusion-detection-systems-Snort-and-Suricata/10.1117/12.2015616.full
% https://www.researchgate.net/profile/David-Day-13/publication/241701294_A_Performance_Analysis_of_Snort_and_Suricata_Network_Intrusion_Detection_and_Prevention_Engines/links/0046351cab8b2bb28d000000/A-Performance-Analysis-of-Snort-and-Suricata-Network-Intrusion-Detection-and-Prevention-Engines.pdf





% Across all regions in Table~\ref{table:data_breakdown}, an average of 20\% of unique scanning IPs and autonomous systems target two neighboring services.
% Scanning traffic exhibits so much target variation, that increasing the raw number of sensors within a network provides significant additional coverage of all unique scanning source IPs within a region; for example, the first 250K IP addresses of the 475K IP addresses (52\%)  of the Orion Network are targeted by 70\% of all unique scanners that target at least one IP addresses within the telescope  (i.e., ``ground truth''). 

% We show in Figure~\ref{fig:uniqueSensor} that across the four regions (Hurricane Electric, \stanford, \merit, and Orion Network Telescope) that contain at least a /26 sub-network of sensors, at least 98\% of all sensors need to be used to obtain 99\% coverage of the network's scanning IP ground truth. 
% %At minimum 77 (30\%) sensor IPs see 50\% of ground truth scanning IPs scanning the Hurricane Electric /24.

% \begin{figure}[h]
%   \includegraphics[width=\linewidth]{fig/unique_sensor_traffic_noOrder.pdf}
%   \caption{\textbf{Unique Sensor Traffic}---% The number of
% 	Across different networks and protocols, each additional sensor IP adds a substantial fraction of unique scanning IPs seen. For example, at minimum 77 (30\%) sensor IPs see 50\% of ground truth scanning IPs scanning a Hurricane Electric /24. 
% 	} \label{fig:uniqueSensor}
% \end{figure}

% Anomaly scanning events that target individual IP addresses dominate coverage of unique scanning IPs, as exhibited by the steps in Figure~\ref{fig:uniqueSensor}.
% For example,  one IP address in Merit networks is targeted by 20\% of all unique scanning IP addresses targeting the /26, with all of the scanning traffic originating from ASN\,6503, Axtel, a Mexican ISP. 



==> tables/neighBits.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{l|cc|l}
\toprule

 Service & \multicolumn{2}{c}{Relative $\sigma$ of \# of malicious scanners} & Stat. Sig  \\
& \multicolumn{2}{c}{ targeting neighborhood} & Increase \\ 
 \cmidrule(r){2-3}
&Same /8 & Different /8 &\\

\midrule
22/SSH & 31\% & 77\% & $+$ \\
23/Telnet & 34\% & 73\% & $+$\\
80/HTTP& 21\% & 25\% & $-$\\
Any/All & 18\% & 40\% & $+$\\ 

% \midrule
% Suricata  & HTTP/80 & \TK &\TK & \TK & \TK& \TK& \TK&$\times$ &$\times$&$\times$ &$\times$  \\
% Accuracy & HTTP/All & \TK & \TK& \TK& \TK& \TK& \TK& $\times$ &$\times$&$\times$ &$\times$  \\

%\midrule
%Top~3 Mal HTTP Payload &  HTTP/All &  - & - &  -&  -& ap-southeast &0.18  &  -&  - 	 \\
\bottomrule \end{tabular}
\quad 

	\caption{\textbf{Attacker Preference Towards Address Spaces}---% Scanning
	There is a significant increase in variance in the number of unique attackers that target neighboring vantage points in different /8 sub-networks compared to in the same /8 network.
	}
\label{table:neighBits}
\end{table}


==> tables/unique_ips_ases.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{llllllll}
\toprule

&
&
\multicolumn{3}{c}{\# of Unique IPs}
&
\multicolumn{3}{c}{\# of Unique ASes}  \\ \cmidrule(r){3-5}\cmidrule(l){6-8}

Network & Collection Method & Average Median & StdDev & Total
 
 & Average Median & StdDev & Total \\

\midrule 

Hurricane Electric & \gn & 5,677 & 0 & 130,103 & 809 & 0 & 8,278   \\
%Alicloud & 4 & 4 & Greynoise \\
AWS & \gn & 2,301 & 324 & 99,566 & 479 & 82 & 7,142\\
Azure & \gn & 212 & 37 & 19,893 & 103 & 14 & 2,477  \\
%Digital Ocean & 2 & 4 & Greynoise \\
Google & \gn & 2,727 & 464 & 103,067 & 565 & 93 & 7,481  \\
%Kametera & 3 & 4 & Greynoise \\
Linode & \gn & 2,814 & 183 & 72,235 & 649 & 64 & 5,984 \\
\midrule
\stanford & Honeytrap & 14,362 & 157 & 105,045 & 1,866 & 29 & 6,177 \\
\merit & Honeytrap & 13,654 & 689 & 106,988 & 1,925 & 29 & 6,315 \\
AWS & Honeytrap & 6,701 & 1,144 & 99,445 & 1,052 & 258 & 7,603 \\
Google & Honeytrap & 9,498 & 3,766 & 109,472 & 1,133 & 211 & 8,431 \\



\bottomrule \end{tabular}
\quad 


\caption{\textbf{Number of unique IPs and ASes targeting each vantage point in a network in one week}--- The average of the median number of distinct scanning IPs per region. \todo{add takeaways of table}
}
\label{table:unique_ips_ases}
\end{table*}



